ShiftAddNet: A Hardware-Inspired Deep Network

Multiplication (e.g., convolution) is arguably a cornerstone of modern deep neural networks (DNNs). However, intensive multiplications cause expensive resource costs that challenge DNNs' deployment on resource-constrained edge devices, driving several attempts for multiplication-less deep networks. This paper presented ShiftAddNet, whose main inspiration is drawn from a common practice in energy-efficient hardware implementation, that is, multiplication can be instead performed with additions and logical bit-shifts. We leverage this idea to explicitly parameterize deep networks in this way, yielding a new type of deep network that involves only bit-shift and additive weight layers. This hardware-inspired ShiftAddNet immediately leads to both energy-efficient inference and training, without compromising the expressive capacity compared to standard DNNs. The two complementary operation types (bit-shift and add) additionally enable finer-grained control of the model's learning capacity, leading to more flexible trade-off between accuracy and (training) efficiency, as well as improved robustness to quantization and pruning. We conduct extensive experiments and ablation studies, all backed up by our FPGA-based ShiftAddNet implementation and energy measurements. Compared to existing DNNs or other multiplication-less models, ShiftAddNet aggressively reduces over 80% hardware-quantified energy cost of DNNs training and inference, while offering comparable or better accuracies. Codes and pre-trained models are available at https://github.com/RICE-EIC/ShiftAddNet.

==> sections/3-Method.tex <==
\section{The Proposed ShiftAddNet}

\textbf{Efficiency Analysis.} 
The well-known hardware practice, shift and add, has the potential to extremely save energy costs.
% FP32 addition cost more 
But previous add based network \cite{chen2019addernet} adopts floating point addition which even cost more than multiplications \cite{bad-add} due to the extra steps of normalising and adding the exponents. 
% fixed point addition is saving
Therefore, quantizing the additive parameters to fixed point format is necessary. For example, when testing 32-bit fixed point operations in 45nm and 0.9V, the energy cost of multiplication is more than 4$\times$ of addition (3.7pJ vs. 0.9pJ) \cite{6757323}.
% shift is also very saving
The shift operations are more hardware friendly, \cite{asati2009comparative} shows for 16-bit architecture, average power and area of multiplications are at least 9.7$\times$ and 1.45$\times$, respectively, of bitwise shift.
The shift range can be further constrained within 6-bit to squeeze more energy savings \cite{elhoushi2019deepshift}.
% shift add can save a lot on hardware resource ---> IoT applications
Hence, substituting multiplication with much cheaper shift and add operations leads to huge amount of energy cost reductions. That is needed for mobile and IoT applications.

\textcolor{red}{This section is NOT a method section. You need to formulate how your network operation and how the trainig process is performed. Plz fix it ASAP if you want to submit}

In this section, we present a multiplication-free DNNs structure for efficient training, termed as \textit{ShiftAddNet}. 
We will first introduce the ShiftAdd layer design, and then study the shift and add components in the deisgned ShiftAdd scheme, respectively.
% and then address \textbf{three key questions} pertraining to the ShiftAddNet: 1) To what extent the multiplication is needed; 2) To what extent larger-grained shift parameter is needed; 3) To what extent smaller-grained add parameter is needed.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/shiftadd_overview-new.pdf}
    \caption{Overview structure of ShiftAddNet.}
    % \textcolor{red}{This is a brainless mistake, why the shift only has one direction???}}
    \label{fig:shiftadd}
\end{figure}


\subsection{ShiftAddNet Overview}

% \begin{minipage}[b]{0.45\linewidth}
Motivated by the hardware expertise that substituting multipliers with shift and add modules saves hardware resources, 
we design a ShiftAdd layer as a building block to consititute ShiftAddNet,
which is dedicated for efficient training and can be widely adopted to substitute the conventional ConvNet. 
As Fig. \ref{fig:shiftadd} shows, ShiftAdd layer consists of two sub-layers: the shift layer and the add layer, where shift layer
% \end{minipage}
% \hfill
% % \begin{minipage}[b]{0.68\linewidth}
% \begin{minipage}[b]{0.52\linewidth}
% \vspace{-0.3em}
% \includegraphics[width=\textwidth]{images/shiftadd.pdf}
% \vspace{-1.3em}
% \captionof{figure}{(a) Multiplicaiton can be substituted by shift and add. (b) Weight structure of ShiftAdd layer.}
% \label{fig:shiftadd}
% \end{minipage}
serves as large-grained feature scaling function and add layer makes further small-grained adjustments to make the ShiftAdd module surjective.
\XH{I think there is no need to talk about ``surjectivity''. I know what you mean -- with add operation we could map input to any real number -- but we need a clearer and more intuitive way to explain it.}

%% shift layer
The weight filters in shift layer only contain powers of 2 parameters,  that can be efficiently encoded and transferred with small bandwidth and can also be expressed as bit-wise shift operations.
The unique weight structure of shift layer ensures the multiplication can be replaced by the low-cost shift operation and therefore achieve aggressive computational and memory-wise efficiency. 
% hardware constraints
Also, considering that the range of dynamic shift linearly related to the hardware resources \cite{gorgin2007reversible}, limiting the hardware efficiency, we aggressively constraint the shift range (e.g., a maximum range of 7 constraints the powers of 2 parameters within $[2^{-7}, 1]$) to meet the efficient training goal.
% \XH{I remember we use larger range for ImageNet experiments.}
% \HR{Here is just a showcase.}
% drawbacks of only shift layer.
However, fully replacing multiplication with shift operation is not enough, because the bit-wise shift is not fully expressive (multiplication by powers of 2) and its range needs to be further constrained for efficient training, which incurs the accuracy drop. 

%% add layer
The add layer is then required to make the function surjective.
\XH{Still I think we don't need surjectivity.}
In particular, we append another add layer behind, which follows the conventional convolution but replace the multiplications with additions.
% \XH{We don't just ``replace multi with add''. That's what AdderNet did. What we propose is to append another add layer after shfit-layer, for adjustment/expressiveness or whatever.}
The additive parameters in add layer should be able to complement the less expressiveness after the large-grained feature scaling in shift layer, which requires wide range of additive parameters.
% training scheme
To achieve the good expressiveness of network,
we follow AdderNet \cite{chen2019addernet} to adopt the improved back-propagation scheme and adaptive learning rate scaling to ensure the sufficient update of additive parameters.
% benefit from shift layer
Benefit from the previous feature scaling in shift layer, the add layer only needs to learn smaller-grained adjustments instead of the fully expressive additive parameters in AdderNet, leaving the room for further pruning to achieve parameter efficiency and making training easier.


% complement each other

Based on the above analysis of each sub-layer, we argue that the shift and add complement each other. Specifically, shift layer provides large-grained feature scaling and add layer further learn small-grained adjustments, 
the proposed ShiftAdd layer can then achieves more flexible control of different levels of granularity in network training as compared to the convolutional layer.
% \XH{Why better granularity than conv layer?}
% \HR{No better granularity but more flexible control.}
% flexible control
Also,
the proposed ShiftAdd layer allows the network to achieve good expressiveness 
% \XH{(I think ``full expressiveness'' is too much)} 
and parameter efficiency, solving the drawbacks of separate shift and add operations.
% The decomposition of multiplications to shift and add operations provides us a flexible control of different levels of granularities in network architecture.
% ShiftAddNet
Finally, we leverage the designed ShiftAdd layer as a building block of ShiftAddNet, aiming at the energy-efficient network training and inference.


\subsection{Study of Shift and Add Components}
The decomposition of multiplication to shift and add provides us a new perspective to explore the network properties in different levels of granularities.
We next study the shift and add components separately to figure out whether the shift layer needs to be trained and whether the add layer is robust to compression, for squeezing more energy efficiency in ShiftAddNet.

\subsubsection{Shift Layer: Learnable versus Fixed}
Motivated by the success of freezing anchor weights \cite{juefei2017local,liu2020orthogonal} for over-parameterized networks, we discuss the weight structure in shift layer and compare the fixed and learnable shift layer.

\textbf{Fixed Shift.} 
% fixed parameters
The shift parameters can be generated stochastically. In particular, we first constraint the shift range and then sample from the 
available 
% \XH{(what does ``sorted'' mean here)} 
powers of 2 within the shift range according to Gaussian distribution, next we sparsify the shift parameters in terms of the given percentage of non-zero weights and randomly assign the signs ($+1$ or $-1$) to the weights with equal probability.
% train
Training a ShiftAddNet with fixed shift layer is straightforward because it doensn't affect back-propagation.
% The error can be back-propagated through the fixed shift layer in the same way they are back-propagated through the learnable shift layer.
However, we can further save the energy cost of ShiftAddNet during training because we can skip the weight gradient calculation.
%the weight will not be updated during training and therefore we do not need to calculate the weight gradients for the fixed shift layer, which further saves the energy cost of ShiftAddNet.

\textbf{Learnable Shift.} 
% learnable parameters
The weight initialization of learnable shift layer is similar with the fixed one, we additionally follow DeepShift\cite{elhoushi2019deepshift} to 1) separate the shift bits and signs and use uniform random distribution to initialize them;
% train
2) adopt the straight through estimator to ignore the rounding effect of shift parameters during network training.
The back-propagation is normally conducted.
Note that we do not need to keep full-precision latent weights during back-propagation, the shift bit will be directly updated when the corresponding gradient is large enough (e.g., $|\mathrm{grad}| > 0.5$) to update the shift bit from $p$ to $p \pm 1$ within the shift range.

% under-parameterized and over-parameterized
Inspired by the success of fixing weights and only learn a proper coordinate system for over-parameterized networks \cite{liu2020orthogonal}, and  fixing spatial convolution in depthwise separable convolution and only train pointwise convolution \cite{juefei2017local}, which are similar with our ShiftAdd layer scheme.
% \XH{Grammar issue.}
We hypothesis that the ShiftAddNet with fixed shift layer can also achieve comparable accuracies,
% \XH{(instead of saying it could achieve SOTA, we can say it provides enough expressiveness/generalizability)} 
or even outperform the default learnable one on IoT applications, because modern DNNs are mostly over-parameterized for these IoT applications of low complexity, fixing the large-grained shift parameters provide a regularization which benefits the training and generalization of such over-parameterized networks \cite{allen2019learning,liu2020orthogonal}.

% While for the larger dataset (e.g., ImageNet), the networks are under-parameterized and therefore fixing the shift layer would perform inferior to the learnable one.


% \begin{itemize}
%     \item Fix shift and train add; benefit; small datasets;
%     \item over-parameterized and under parameterized scenarios.
% \end{itemize}

% Inspired by the success of freezing spatial convolution in depthwise separable convolution \cite{juefei2017local}, fixing weights and only learn a proper coordinate system for over-parameterized networks.

 
 % We argue that the shifting layers can provide great generalization ability to the model if they are properly initialized, even when they are barely trained or totally fixed. This property leads to significant reduction in energy and latency because the the parameters in the shifting layers can be directly hard-coded into the hardware and require little dynamical changes. To relieve the potential model capacity loss, we cascade shifting layers with the adding layers which offer the model more learning capability to fit the data without bringing too much computational and memory overheads.
 
\subsubsection{Add Layer: Full-precision versus Compressed}
% \begin{itemize}
%     \item why we need to quantize and sparsify it
%     \item shift layer helps to alleviate quantization effects.
%     \item shift layer helps to alleviate sparsification effects.
% \end{itemize}

\textbf{The Necessity for Quantizing Add Layer.} Addition need to be quantized to fixed point to show the efficiency, otherwise the floating point addition cost more than multiplication.
Specifically, when two real numbers are added, the mantissa of the smaller number must be first shifted to make sure the exponents match (a process termed normalisation) \cite{FP-adder}, which requires complex control logic in hardware design and shows even worse energy efficiency than multiplication \cite{bad-add}, limiting the benefits of add-based networks. Therefore, quantizing the additive parameters to fixed point is necessary to meet the efficient training goal.

\textbf{Compress Add Layer.}
% Difficulties for compressinv add layer
AdderNet \cite{chen2019addernet} fully replaces the multiplications in DNNs with additions, but such add-only network is not parameter efficient as compared to multiplication-based ConvNet, so that the add layer is not robust to the further pruning or quantization of the additive parameters.
% since it has less efficiency than multiplication \XH{(this is not what parameter inefficiency means. it's the outcome of this inefficiency)}. 
For example, modern DNNs need lots of feature scaling which can be easily achieve by multiplication while requires large amount of additive parameters at different scales. Compressing the inefficient add layer does harm to the network performance.

% Shift Layer Favors the Parameter Efficiency in Add Layer
However, the shift layer can help to alleviate the difficulties in compressing the add layer. In particular, the shift layer provides large-grained feature scaling to meet the inefficiency in additive parameters, in which way add layer only need additive parameters to learn small-grained adjustments, making the room for further quantization and pruning and easing the network training.

% \subsection{To What Extent Multiplication Is Needed?}

% % refer to hardware expertise to justify

% Instead of designing efficient modules, like depth-wise convolution, to reduce the numbers of multiplication. We here rethink totally replacing multiplication with cheaper shift or add operations, where shift operation can be seen as constrained multiplication with powers of 2.

% \textbf{Constrained multiplication is not enough.}
% \begin{itemize}
%     \item spatial shift requires point-wise convolution
%     \item bit shift has coarse granularity, also the shift range need to be constrained to meet the efficient training goal, which will degrade the accuracy.
% \end{itemize}

% \textbf{Add-based networks lack the flexibility of multiplication.}
% \begin{itemize}
%     \item addition need to be quantized to show the efficiency, otherwise it cost more than multiplication. However, add only network are not robust to quantization.
%     \item add only network is not parameter efficient, it requires large amount of additive patterns, which are hard to train and not robust to pruning.
% \end{itemize}

% Combining shift and add can be a substitution to multiplication without lose the generality and also provide flexible control to network training in different granularities.

% Next we will further explore the flexible control of network training and the potential efficiency to meet efficient training goal in the ShiftAdd scheme.

% Observation/conclusion: trade-off between the energy efficiency and accuracy. The reasonable shift range should be xxx to meet the efficient training goal while maintaining the decent accuracy.

% \subsection{To What Extent Larger-Grained Shift Operation Is Needed?}

% \textbf{Fix shift and train add.} We fix the random-initialized parameters in shift layer and only train the add layer. It works for small datasets like CIFAR. Since modern DNNs are over-parameterized, and therefore leaving enough room for fixing the larger-grained parameters during training. While for larger dataset like ImageNet, ... 

% \textbf{Sparsity in fixed shift layers.} Sparsity in shift layer will not degrade the final accuracy while high sparsity will hinder the convergence speed.

% Conclusion: Fixing shift layer can also lead to SOTA results in small datasets while ... in under-parameterized scenario. 



% \subsection{To What Extent Smaller-Grained Add Operation Is Needed?}

% \textbf{Sparsity in add layer.} Keep fixing the shift parameters, and further sparsify the adding residual patterns.

% \textbf{Quantize add parameters.}

% Furthermore, adding small sparsity in add layer while keeping fixed shift parameters can also maintain decent accuracy and show better robustness than add only network.


% To investigate whether the ShiftAdd networks with fixed shift parameters generalize well to the under-parameterized scenario, ...

